Robust and Efficient Imbalanced Positive-Unlabeled Learning with Self-supervision

Learning from positive and unlabeled (PU) data is a setting where the learner only has access to positive and unlabeled samples while having no information on negative examples. Such PU setting is of great importance in various tasks such as medical diagnosis, social network analysis, financial markets analysis, and knowledge base completion, which also tend to be intrinsically imbalanced, i.e., where most examples are actually negatives. Most existing approaches for PU learning, however, only consider artificially balanced datasets and it is unclear how well they perform in the realistic scenario of imbalanced and long-tail data distribution. This paper proposes to tackle this challenge via robust and efficient self-supervised pretraining. However, training conventional self-supervised learning methods when applied with highly imbalanced PU distribution needs better reformulation. In this paper, we present \textit{ImPULSeS}, a unified representation learning framework for \underline{Im}balanced \underline{P}ositive \underline{U}nlabeled \underline{L}earning leveraging \underline{Se}lf-\underline{S}upervised debiase pre-training. ImPULSeS uses a generic combination of large-scale unsupervised learning with debiased contrastive loss and additional reweighted PU loss. We performed different experiments across multiple datasets to show that ImPULSeS is able to halve the error rate of the previous state-of-the-art, even compared with previous methods that are given the true prior. Moreover, our method showed increased robustness to prior misspecification and superior performance even when pretraining was performed on an unrelated dataset. We anticipate such robustness and efficiency will make it much easier for practitioners to obtain excellent results on other PU datasets of interest. The source code is available at \url{https://github.com/JSchweisthal/ImPULSeS}

==> chapters/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the %code and datasets? \answerYes{See %Section~\ref{gen_inst}.}
%  \item Did you include the license to the %code and datasets? \answerNo{The code and %the data are proprietary.}
%  \item Did you include the license to the %code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only %use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{\textbf{see Section~\ref{sec:intro} and abstract}}
    
  \item Did you describe the limitations of your work?
    \answerYes{\textbf{see Section~\ref{sec:impact-limitations}}}
  
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{\textbf{see Section~\ref{sec:impact-limitations}}}
    
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{\textbf{See Section~\ref{sec:theory}}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{\textbf{In appendix~\ref{appendix}}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{\textbf{As a ZIP in the supplementary}}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{\textbf{See Sections \ref{sec:experiments}, \ref{sec:results}, and \ref{sec:ablation}}}
    
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{\textbf{All reported results are averaged over three runs.}}
    

        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{\textbf{see Section\ref{sec:experiments}}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{see Read.me of code}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
     \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
     \answerNA{}
\end{enumerate}


\end{enumerate}


==> chapters/results-old.tex <==
\section{Results}
% in general CIFAR10, and CIFAR100 results, 
% 2class cifar10 maye just in secon method? (but selfsupervised important becaue of mlti positive learning)
% glaucoma not sure, bad results , fuzzy data, either as limitation of method or appendix
% confusion matrix

% reducing risk of overfitting because of just linear classification head --> solve problem of too high flexibility for unbaised pu learning, nnpu maybe note really needed --> explained in prior robsutness part, but maybe also do chart here?
In the following, we describe the performance of our framework under different scenarios, hereafter referred to as ImPULSeS.
As a comparison method, in the following called \textit{imbnnPU}, we used the loss $\mathcal{L}_{imbnnPU}$ of \cite{su2021positive} for training a model without pretraining and without decoupling feature extractor and classifier, as our method does.
For comparability, we also used ResNet-50 as the backbone for this model, which means that in both methods the final model had the same number of parameters, and follow the same optimization settings from subsection \ref{ssl:subsec_optim}.

\subsection{Classification Performance}
Table \ref{tab:self_results} shows the results of our method debiased+imbnnPU on the test datasets.
For the artificially generated imbalanced PU datasets CIFAR-10 and CIFAR-100, our method clearly achieved better results in terms of accuracy, F1-score and AUC of the test dataset compared to the simple ResNet-50 model with imbnnPU loss without pretraining.
For CIFAR-10 there are performance improvements of 8.8\%, 11.0\% and 5.4\%, for CIFAR-100 2.4\%, 18.5\% and 12.7\%.
For CIFAR-100, the test data set was imbalanced, so the accuracy and the minor improvement of only 2.4\% should not be overvalued because it does not adjust for the different number of samples per class.

In addition, for CIFAR-10 we performed the pre-training with the original NT-Xent loss used in SimCLR instead of the debiased loss, with the same settings.
In comparison to NT-Xent, the debiased loss achieved an improvement of 1-1.5 percentage points in the metrics.

For Glaucoma, however, we observed hardly any differences in performance between models with and without pretraining.
This suggests that in the self-supervised pretraining no additional information helpful for classification was stored in the representations, but at the same time decoupling did not degrade performance.
It should be noted that the used self-supervised architecture of \cite{chen2020simple} with choice of image augmentations was optimized for typical benchmark datasets such as CIFAR-10 and CIFAR-100, while the transferability to other datasets with different underlying structures, like in medical imaging, is not ensured.
\newline
% task of imbalanced and pu
% table and explain the table
% compare with fully supervised model
\begin{table}[ht] %TABLE COMPETITORS
\centering
% \begin{tabular}{ p{3cm}||p{1.5cm}|p{1.5cm}|p{1.5cm} }
\begin{tabular}{ l c c c c}
\toprule
% \multicolumn{4}{c}{} \\
%  \hline
   Dataset &  Method & Accuracy & F1 & AUC\\
  \cmidrule{1-2} \cmidrule(l){3-5}
%   & \multicolumn{3}{|c}{Random Walk 1} \\
 \multirow{3}{*}{CIFAR-10} &   imbnnPU  & 86.5 & 83.0 & 93.6\\
 &  NT-Xent + imbnnPU    & 94.3 & 92.5 & 97.9\\
  &  ImPULSeS    & \textbf{95.3} & \textbf{94.0} & \textbf{99.0}\\
  \cmidrule{1-2} \cmidrule(l){3-5}
%  \hline
%   & \multicolumn{3}{|c}{Random Walk 2} \\
 \multirow{2}{*}{CIFAR-100} & imbnnPU  & \textit{86.7} & 44.1 & 82.9\\
  &  ImPULSeS & \textbf{\textit{89.1}} & \textbf{62.6} & \textbf{95.6}\\
  
  \cmidrule{1-2} \cmidrule(l){3-5}
  
  \multirow{3}{*}{Glaucoma} & imbnnPU  & \textbf{75.0} & 67.0 & 77.7\\
&  NT-Xent + imbnnPU    & 74.6 & 67.3 & \textbf{77.8} \\
  &  ImPULSeS    &  74.2 & \textbf{68.3} & 77.3\\
 \bottomrule
\end{tabular}
 \caption[Results of self-supervised pre-training for imbalanced PU learning.]{\label{tab:self_results}Results of self-supervised pre-training for imbalanced PU learning vs. imbalanced PU learning without pre-training. Best performances per dataset and measure are \textbf{bold}.}
\end{table}

\subsection{Competitors}
In PU learning, there are only few approaches so far that focus on the application to imbalanced data with few positive samples. 
\cite{su2021positive} showned that their imbalanced nnPU loss outperformed many other methods in this setting, such as \textit{nnPU} \citep{kiryo2017positive}, \textit{self-PU} \citep{chen2020self}, \textit{SMOTE} \citep{chawla2002smote}, or \textit{SSImbalance} \citep{yang2020rethinking}. 

For the usual balanced scenario, there are some state-of-the-art methods that report their results for CIFAR-10 trained on the full train dataset with the approximately balanced split ``vehicles'' : ``animals'' with ratio $2:3$, but they are not explicitly suitable for imbalanced learning.
Since our debiased+imbnnPU method, as described above, far outperformed the simple ResNet-50 with imbnnPU method, we wanted to check whether this two-step architecture with pre-training and a separate classifier can achieve similar performances to current SOTA-PU methods even when training on less data overall and with class imbalance. 

As comparison methods, we select \textit{VPU} \citep{chen2020variational}, \textit{PAN}\citep{hu2021predictive}, \textit{Self-PU} \citep{chen2020self} and \textit{PUUPL} \citep{dorigatti2022positive} and use the performance reported in the articles for CIFAR-10 on the same class split ``vehicles'' vs. ``animals''.
Here, all 20,000 samples of the positive ``vehicles'' class are used for training or validation, of which 3,000 (or 1,000) are known to be labeled, whereas we use only 3,000 positive samples in total with 600 labeled.
The test dataset remains the same in both scenarios.

Table \ref{tab:competitors} shows the accuracy of the competitors.
Our method clearly surpasses the other baselines, and can improve the accuracy by 3.9 percentage points compared to the previous best method PUUPL.
Moreover, we only need 66\% of the train samples, 15\% of the positive samples, and 20\% of the labeled samples that PUUPL uses.

\begin{table}[ht] %TABLE COMPETITORS
\centering
% \begin{tabular}{ p{3cm}||p{1.5cm}|p{1.5cm}|p{1.5cm} }
\begin{tabular}{ c c c c c}
% \multicolumn{4}{c}{} \\
%  \hline
\toprule
%  Method & Train Samples & Positives Labeled & Accuracy\\
%  \cmidrule{1-1}\cmidrule(l){2-3}\cmidrule(l){4-4}
%%   & \multicolumn{3}{|c}{Random Walk 1} \\
%
%VPU & 50,000 & 3,000 & 89.5 \\
%PAN & 50,000 & 1,000 & 89.7 \\
%Self-PU & 50,000 & 3,000 & 90.8 \\
%PUUPL & 50,000 & 3,000 & 91.4 \\
%  \cmidrule{1-1}\cmidrule(l){2-3}\cmidrule(l){4-4}
%imbnnPU & \textbf{33,000} & \textbf{600} & 86.5 \\
%\textbf{ImPULSeS} & \textbf{33,000} & \textbf{600} & \textbf{95.3} \\
Method & Labeled P. & Train P. & Tot. Train & Accuracy \\
\cmidrule{1-1}\cmidrule(l){2-4}\cmidrule(l){5-5}
VPU & 3,000 & 20,000 & 50,000 & 89.5 \\
PAN & 1,000 & 20,000 & 50,000 & 89.7 \\
Self-PU & 3,000 & 20,000 & 50,000 & 90.8 \\
PUUPL & 3,000 & 20,000 & 50,000 & 91.4 \\
\cmidrule{1-1}\cmidrule(l){2-4}\cmidrule(l){5-5}
imbnnPU & \textbf{600} & \textbf{3,000} & \textbf{33,000} & 86.5 \\
ImPULSeS & \textbf{600} & \textbf{3,000} & \textbf{33,000} & 95.3 \\
\bottomrule
\end{tabular}
\caption[Performance of competitors trained on balanced CIFAR-10.]{\label{tab:competitors} Performance of SOTA-competitors trained on balanced PU CIFAR-10. Best performance and fewest resources needed are \textbf{bold}.}
\end{table}
% cite all the esults and papers!!!

% --> great performance compared to imbnnpu on resnet50
% --> compare to competitiors using a) whle cifar10, b) more labeled data (1000 - 3000) c) different architecture
% --> include probabaly ablation (simclr + bce, nnpu, maybe upu..)

\subsection{Comparison to supervised baseline}
The loss $\mathcal{L}_{imbnnPU}$ \eqref{eq:imbnnpu} that we used for our experiments actually tries to minimize the empirical risk on the underlying true binary classification problem with the true label $y$ by reweighting and reformulating the loss on the PU scenario using the PU label $s$ and adjusting for imbalance.
Consequently, the performance of a model with the same architecture trained on the true positive and negative labels can be viewed as an upper bound on the performance we are trying to achieve.

To investigate how close our framework comes to this upper bound and whether pre-training can be helpful to reduce the gap between PU and fully supervised performance, we trained both models in a supervised setting on the true labels using a weighted binary cross-entropy (wBCE) loss on the predictions $\hat{y}$:
\begin{equation}
\mathcal{L}_{wBCE}(\hat{y}, y)=w_{pos} y_{i}  \log (\hat{y})
+(1-y_{i}) \log (1-\hat{y})
\end{equation}
where $w_{pos}$ is the weight of the positive samples and is set to the ratio of number of negatives to number of positives in the training dataset.

The performances of the supervised models on both methods are displayed in Table~\ref{tab:self_PUvsSup}.
The debiased+wBCE variant achieved better results than training with the wBCE loss from scratch.
Notably, the gap between PU learning and fully supervised learning is almost closed by our use of pretraining.
For example, the difference in F1-score and AUC for CIFAR-10 (CIFAR-100) with pretraining was 0.9\% and 0.4\% (4.2\% and 1.5\%), whereas without pretraining the difference was 5.3\% and 3.2\% (9.2\% and 5.3\%).
This suggests that self-supervised pretraining is not only beneficial to tackle the problem of class imbalance, but also reduces the performance gap between PU and PN data.

\begin{table}[ht]
\centering
\begin{tabular}{ c c c c c c}
  \toprule
 Dataset & Labels &  Method & Acc. & F1 & AUC\\
  \cmidrule(r){1-3}\cmidrule{4-6}
 \multirow{4}{*}{CIFAR-10} & \multirow{2}{*}{PU} &   imbnnPU  & 86.5 & 83.0 & 93.6\\
  & & ImPULSeS    & \textbf{95.3} & \textbf{94.0} & \textbf{99.0} \\
  \cmidrule(r){2-3}\cmidrule{4-6}
  &  \multirow{2}{*}{PN} &   wBCE  & 91.0 & 88.3 & 96.8\\
  & & debiased + wBCE   & \textbf{95.9} & \textbf{94.9} & \textbf{99.4}  \\
  \cmidrule(r){1-3}\cmidrule{4-6}
 \multirow{4}{*}{CIFAR-100} & \multirow{2}{*}{PU} &  imbnnPU  & \textit{86.7} & 44.1 & 82.9\\
  & & ImPULSeS    & \textbf{89.1} & \textbf{62.6} & \textbf{95.6} \\
  \cmidrule(r){2-3}\cmidrule{4-6}
  &  \multirow{2}{*}{PN} &   wBCE  & \textit{91.0} & 53.3 & 88.2\\
  & & debiased + wBCE   & \textbf{91.7} & \textbf{68.8} & \textbf{97.1} \\
  \bottomrule
\end{tabular}
 \caption[Performance with and without debiased pre-training for PU vs. supervised data.]{\label{tab:self_PUvsSup}Performance with and without debiased pre-training for PU and fully-supervised (PN) labeled data. Best performance in \textbf{bold}.}
\end{table}

\subsection{Quality of Learned Representations}
The main feature of ImPULSeS compared to the competitors is that representation learning is decoupled from the actual classification task.
In the second step, ImPULSeS uses the same architecture as the imbnnPU baseline, except that the latter starts training from scratch whereas our method only fine-tunes the weights in the last layer, while keeping the previous layers frozen.
Since our method achieved much better results in the evaluation, the quality of the representation before the last linear layer was obviously significant for the quality of the classifier. 

% figure ala imbalanced medical here
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.9\linewidth} 
      \includegraphics[width=\linewidth]{figures/tsne_cifar10_imbalancednnPU.png} 
   \end{subfigure} %\hfill% 
    \begin{subfigure}[t]{0.9\linewidth} 
      \includegraphics[width=\linewidth]{figures/tsne_cifar10_debiased.png} 
   \end{subfigure} %\hfill% 
   \caption[t-SNE visualization of representations of self-supervised pre-training.]{t-SNE visualization of representations on test dataset of CIFAR-10. Top: ResNet-50 trained on imbalanced nnPU loss without pre-training. Bottom: After pre-training on debiased contrastive loss. Color-coded for underlying 10 subclasses (left) and binary classes (right).}
   \label{fig:tsne_10_imbnnpu} 
\end{figure}


Figure \ref{fig:tsne_10_imbnnpu} shows the t-SNE \citep{van2008visualizing} visualizations of the 2048-dimensional representations of the test dataset of CIFAR-10 of both models.
Even though the debiased pretraining was completely unsupervised, it resulted in representations that more clearly separated positives and negatives compared to training a classifier from scratch using the imbalanced nnPU loss.
Such representations even separated the different classes found in the original dataset, unlike those resulting from the imbalanced nnPU loss that were oblivious to such latent structures.
Explicitly representing these substructures makes it then considerably easier to identify the unlabeled positive samples even when very little labeled examples are provided.
It is for this reason that decoupling representation learning from classifier learning was found to indeed improve the final classification performance \citep{kang2019decoupling}, and the robustness of contrastive self-supervised pretraining on imbalanced data has been well studied \citep{yang2020rethinking}, \citep{liu2021self}.
This principle is also found in few-shot learning \citep{wang2020generalizing}, where a classifier is also trained using representation learning and few labeled data.
Our contribution is to show that this robustness is also highly beneficial for PU learning.

\begin{table}[ht]
\centering
\begin{tabular}{c c c c}
\toprule
Pretraining & Loss & Accuracy & F1 \\
\cmidrule(r){1-2}\cmidrule{3-4}
\multirow{4}{*}{SimCLR}
& BCE & 60.05 & 0.25 \\
& wBCE & 94.17 & 92.4 \\
\cmidrule(r){2-2}\cmidrule{3-4}
& nnPU & 93.09 & 90.74 \\
& imbnnPU & \textbf{94.26} & \textbf{92.50} \\
\cmidrule(r){1-2}\cmidrule{3-4}
\multirow{4}{*}{Debiased SimCLR}
& BCE & 60.03 & 0.15 \\
& wBCE & 95.27 & \textbf{94.11} \\
\cmidrule(r){2-2}\cmidrule{3-4}
& nnPU & 92.75 & 90.20 \\
& imbnnPU & \textbf{95.29} & 94.05 \\
\bottomrule
\end{tabular}
\caption{Comparison between PU losses and (weighted) binary cross-entropy (BCE) treating unlabeled as negatives on the imbalanced CIFAR-10 dataset.}
\label{tbl:bcevspu}
\end{table}

Such high quality representations already separating classes in the latent space raise the question of whether a PU loss is needed at all.
We thus trained a classifier using the BCE loss and treating all unlabeled as negative samples.
While the equally-weighted BCE failed to learn any signal and collapsed to all-negative predictions due to the data imbalance, the weighted BCE performed better than the nnPU loss and was very competitive with the imbalanced nnPU loss.
The use of the debiased SimCLR pretraining further increased performance by about one percentage point (Table~\ref{tbl:bcevspu}).

\subsection{Robustness Against Mis-specification of the Class Prior}
% include charts of runs for overnnpu vs impulses with differnt priors here: ciafr10 imbalanced, not 10 times prior, results either accuracy or f1 score (maybe even auc?) to show that it's even a better reanking funtion, not a better decision boundary

In the previous analyses, we always assumed the class prior $\pi$ to be known, and in the imbnnPU loss for each dataset to be set to the proportion of positive samples in the unlabeled samples, following \cite{su2021positive} and \cite{kiryo2017positive}.
In real-world applications, however, this proportion is often not known and must be estimated using domain knowledge or other methods, and imperfect estimation can degrade the final classification performance.
In the following, we thus investigate how misspecification of $\pi$ in $\mathcal{L}_{imbnnPU}$ changes the performance of the model.

Both accuracy and F1-score depend strongly on the decision boundary, which is shifted according to the chosen class prior.
The monotony of the score $g$ is however unaffected by the setting of $\pi$, and thus the model could still be suitable as a ranking model.
It is for this reason that the AUC proved to be a reliable performance metric for model selection under such settings as PU learning as well as learning with noisy labels \citep{pmlr-v37-menon15,Jain_White_Radivojac_2017}.


\subsection{Robustness due to representations}

\subsubsection{prior}
In figure \ref{fig:priormis}, the course of the AUC on the test dataset of CIFAR-10 is displayed over the 100 training epochs of the PU classifier with distorted priors for both imbnnPU and ImPULSeS .
We performed one run for each distortion factor $b_{dis}$ of the true prior $\pi$, so that in each case the prior $\pi$ was replaced by the distorted prior $\pi_{dis}=b_{dis}\cdot \pi$.
Here, $b_{dis}$ varies from 0.1 to 10.0, with 1.0 yielding the model with the correct $\pi$. 

In general, our method had higher AUC than the model without self-supervised pretraining even under different misspecified priors.
The variance was also smaller and the learning curve more stable, since only the weights of the classifier and not the entire ResNet-50 parameters were trained.
For both models, no deterioration of the performance was observed when underestimating $\pi$, likely because the portion of positives was already very low.
When overestimating $\pi$, a deterioration could be observed for both models starting at $b_{dis}\geq5$, although the performance decrease of our method was less marked.
At extreme overestimation levels of $b_{dis}=10$, strong deviations in stability occurred for both methods and the AUC of our model even decreased in the course of training.
At the same time, the initial AUC was above 95\% owing to the high-quality representations learned during pretraining, which do not need the parameter $\pi$.
In conclusion, even with strong misspecification of the class prior, high stability and performance were achieved by our framework.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/self_priormis_auc.png} 
   \caption[Robustness against prior mis-specification.]{Robustness against prior mis-specification for different distortion factors $b_{dis}$ of the prior. AUC of the test dataset of CIFAR-10 is plotted over 100 training epochs for imbnnPU (left) and for the classifier of debiased+imbnnPU after finished pre-training (right).}
   \label{fig:priormis} 
\end{figure}

\subsubsection{pretraining dataset}
here we show that one can pretrain on different datasets (imagenet) and still get superior performance in PU classification
especially cool since pretrained imagenet models are easy to get
this makes it very efficient to train a PU classifier on a new dataset

==> tables/balance.tex <==
\begin{table}[ht] %TABLE COMPETITORS
\centering
\begin{tabular}{ l c c c}
\toprule
   Method &  Accuracy & F1 & AUC\\
  \cmidrule{1-1} \cmidrule(l){2-4}
 \multirow{1}{*}{SimCLR} 
  & {60.0} & {0.14} & {99.31}\\
  \cmidrule{1-1} \cmidrule(l){2-4}
 \multirow{1}{*}{DebiasedContrastive} 
  & {60.0} & {0.22} & {99.38}\\
    \cmidrule{1-1} \cmidrule(l){2-4}
 \multirow{1}{*}{ImPULSeS} 
  & \textbf{\textbf{97.15}} & \textbf{96.41} & \textbf{99.40}\\
 \bottomrule
\end{tabular}
 \caption[]{\label{tbl:balanced} Comparison of performance on balanced PU dataset. Best performance in \textbf{bold}.}
\end{table}


==> tables/finetunlosses.tex <==
%---------------------------------------------------
%     Table Linear Evaluation 
%---------------------------------------------------

\begin{table}[ht] %TABLE COMPETITORS
\centering
\begin{tabular}{ l c c c c}
\toprule
   Dataset &  Method & Accuracy & F1 & AUC\\
  \cmidrule{1-2} \cmidrule(l){3-5}
 \multirow{3}{*}{CIFAR-10} 
  &  SimCLR~\cite{chen2020self}                     & xx & xx & xx\\ 
  &  Debiased contrastive~\cite{chuang2020debiased} & xx & xx & xx\\ 
  &  PUUPL~\cite{dorigatti2022positive}             & xx & xx & xx\\   
  &  VPU~\cite{}                                    & xx & xx & xx\\ 
  &  Self-PU~\cite{chen2020self}                    & xx & xx & xx\\ 
  &  Oversampled-nnPU~\cite{su2021positive}         & 86.5 & 83.0 & 93.6\\
  &  ImPULSeS & \textbf{95.3} & \textbf{94.0} & \textbf{99.0}\\
  \cmidrule{1-2} \cmidrule(l){3-5}
 \multirow{2}{*}{CIFAR-100} 
  &  SimCLR~\cite{chen2020self}                    & xx & xx & xx\\ 
  &  Debiased contrastive~\cite{chuang2020debiased} & xx & xx & xx\\ 
  &  PUUPL~\cite{dorigatti2022positive}             & xx & xx & xx\\   
  &  VPU~\cite{}                                    & xx & xx & xx\\ 
  &  Self-PU~\cite{chen2020self}                    & xx & xx & xx\\ 
  &  Oversampled-nnPU~\cite{su2021positive}         & \textit{86.7} & 44.1 & 82.9\\ 
  &  ImPULSeS & \textbf{\textit{89.1}} & \textbf{62.6} & \textbf{95.6}\\
  \cmidrule{1-2} \cmidrule(l){3-5}
  \multirow{3}{*}{Glaucoma} 
  & SimCLR~\cite{chen2020self}                    & xx & xx & xx\\ 
  & Debiased contrastive~\cite{chuang2020debiased} & xx & xx & xx\\ 
  & PUUPL~\cite{dorigatti2022positive}             & xx & xx & xx\\   
  & VPU~\cite{}                                    & xx & xx & xx\\ 
  & Self-PU~\cite{chen2020self}                    & xx & xx & xx\\ 
  & Oversampled-nnPU~\cite{su2021positive}   & \textbf{75.0} & 67.0 & 77.7\\
  & ImPULSeS    &  74.2 & \textbf{68.3} & 77.3\\
 \bottomrule
\end{tabular}
 \caption[]{\label{tab:self_results}Imbalanced Positive-Unlabeled classification performance comparison. The best score for each metric is printed \textbf{bold}.}
% \caption[Results of self-supervised pre-training for imbalanced PU learning.]{\label{tab:self_results}Results of self-supervised pre-training for imbalanced PU learning vs. imbalanced PU learning without pre-training. Best performances per dataset and measure are \textbf{bold}.}
\end{table}
